Quantifying the Generation Modality Gap in Speech-Text Language Models

Pure speech language models often lag behind text and speech-text language models in generating coherent content, but this gap is difficult to quantify because speech and text systems are typically evaluated with different metrics and trained on different data. We study the speech-text modality gap in a family of spoken language models, based on flow matching for continuous acoustic feature generation. We construct a unified generation-based evaluation suite that compares speech-only, text-only, and speech-text language models trained on matched data distributions and evaluated in matched generation settings. We evaluate generated continuations along multiple dimensions: semantic coherence, measured by transcribing generated speech and scoring it with a reference language model; local phonetic structure, measured by phone n-gram distributional statistics; speaker consistency and acoustic quality; and emotion-based distributional metrics. Across datasets, we find that joint speech-text modeling substantially improves semantic coherence. However, the improvement is not uniform across metrics: phone-level metrics change only modestly, speaker similarity and predicted quality are lower for speech-text continuations, while emotion-based distributional metrics improve. Compared with larger-scale speech-only models, our speech-text model closes much of the scaling gap in transcript-based semantic coherence, suggesting that text provides an efficient semantic training signal for spoken language modeling.

==> all_table.tex <==
% Requires \usepackage{booktabs,multirow,graphicx}
\begin{table}[H]
\centering
\caption{Detailed metrics for each model across training datasets and prompt sets. Parameter counts exclude the input embedding layer.}
\label{tab:detail}
\renewcommand{\arraystretch}{1.08}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllcrrrrrrrrrrrr@{}}
\toprule
 &  &  &  & \multicolumn{4}{c}{C4 prompts (4707/7500)} & \multicolumn{4}{c}{Emilia prompts (4733/7500)} & \multicolumn{4}{c}{Libri prompts (4710/7500)} \\
\cmidrule(lr){5-8}\cmidrule(lr){9-12}\cmidrule(lr){13-16}
Model & Training data & Variant & Params. & genPPL $\downarrow$ & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ & genPPL $\downarrow$ & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ & genPPL $\downarrow$ & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ \\
\midrule
\midrule
\multirow{6}{*}{Flow-based} & \multirow{2}{*}{C4} & Speech-only & 456M & 228.8 & 0.47 & 0.70 & 3.41 & 265.1 & 0.52 & 0.36 & 3.28 & 291.6 & 0.56 & 0.42 & 3.35 \\
 &  & Speech-text & 456M & 49.9 & 0.47 & 0.62 & 3.09 & 51.8 & 0.51 & 0.26 & 2.90 & 63.4 & 0.53 & 0.32 & 3.02 \\
\addlinespace[2pt]
 & \multirow{2}{*}{Emilia10k} & Speech-only & 456M & 223.5 & 0.54 & 0.44 & 3.34 & 183.3 & 0.51 & 0.47 & 3.19 & 195.8 & 0.56 & 0.40 & 3.12 \\
 &  & Speech-text & 456M & 81.8 & 0.53 & 0.36 & 3.23 & 52.9 & 0.50 & 0.41 & 3.07 & 78.7 & 0.55 & 0.33 & 3.04 \\
\addlinespace[2pt]
 & \multirow{2}{*}{MLSEn10k} & Speech-only & 456M & 220.7 & 0.57 & 0.53 & 3.43 & 198.0 & 0.55 & 0.42 & 3.22 & 160.0 & 0.50 & 0.49 & 3.23 \\
 &  & Speech-text & 456M & 92.4 & 0.54 & 0.39 & 3.12 & 80.9 & 0.54 & 0.29 & 2.82 & 63.4 & 0.49 & 0.36 & 2.86 \\
\midrule
\multirow{3}{*}{Llama-Mimi} & Emilia10k & Matched reproduced & 241M & 407.9 & 0.52 & 0.40 & 3.10 & 283.0 & 0.50 & 0.45 & 3.14 & 328.3 & 0.55 & 0.38 & 2.94 \\
 & \multirow{2}{*}{240k h speech} & \multirow{2}{*}{Published} & 973M & 106.8 & 0.52 & 0.48 & 3.07 & 86.5 & 0.50 & 0.46 & 2.93 & 80.0 & 0.47 & 0.44 & 2.92 \\
 &  &  & 7.54B & 68.3 & 0.51 & 0.49 & 3.03 & 53.0 & 0.50 & 0.48 & 2.90 & 48.7 & 0.47 & 0.45 & 2.92 \\
\bottomrule
\end{tabular}%
%}
\end{table}


==> all_table_vertical.tex <==
\begin{table}[H]
\centering
\caption{Detailed metrics for each model across training datasets and prompt sets. Parameter counts exclude the input embedding layer.}
\label{tab:detail}
\renewcommand{\arraystretch}{1.08}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllcrrrr@{}}
\toprule
Model & Training data & Variant & Params. & Prompt set & genPPL $\downarrow$ & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ \\
\midrule
\midrule

\multirow{18}{*}{Flow-based}
& \multirow{6}{*}{C4}
& \multirow{3}{*}{Speech-only}
& \multirow{3}{*}{456M}
& C4 (4707/7500) & 228.8 & 0.47 & 0.70 & 3.41 \\
& & & & Emilia (4733/7500) & 265.1 & 0.52 & 0.36 & 3.28 \\
& & & & Libri (4710/7500) & 291.6 & 0.56 & 0.42 & 3.35 \\
\cmidrule(lr){3-9}
& & \multirow{3}{*}{Speech-text}
& \multirow{3}{*}{456M}
& C4 (4707/7500) & 49.9 & 0.47 & 0.62 & 3.09 \\
& & & & Emilia (4733/7500) & 51.8 & 0.51 & 0.26 & 2.90 \\
& & & & Libri (4710/7500) & 63.4 & 0.53 & 0.32 & 3.02 \\

\addlinespace[2pt]

& \multirow{6}{*}{Emilia10k}
& \multirow{3}{*}{Speech-only}
& \multirow{3}{*}{456M}
& C4 (4707/7500) & 223.5 & 0.54 & 0.44 & 3.34 \\
& & & & Emilia (4733/7500) & 183.3 & 0.51 & 0.47 & 3.19 \\
& & & & Libri (4710/7500) & 195.8 & 0.56 & 0.40 & 3.12 \\
\cmidrule(lr){3-9}
& & \multirow{3}{*}{Speech-text}
& \multirow{3}{*}{456M}
& C4 (4707/7500) & 81.8 & 0.53 & 0.36 & 3.23 \\
& & & & Emilia (4733/7500) & 52.9 & 0.50 & 0.41 & 3.07 \\
& & & & Libri (4710/7500) & 78.7 & 0.55 & 0.33 & 3.04 \\

\addlinespace[2pt]

& \multirow{6}{*}{MLSEn10k}
& \multirow{3}{*}{Speech-only}
& \multirow{3}{*}{456M}
& C4 (4707/7500) & 220.7 & 0.57 & 0.53 & 3.43 \\
& & & & Emilia (4733/7500) & 198.0 & 0.55 & 0.42 & 3.22 \\
& & & & Libri (4710/7500) & 160.0 & 0.50 & 0.49 & 3.23 \\
\cmidrule(lr){3-9}
& & \multirow{3}{*}{Speech-text}
& \multirow{3}{*}{456M}
& C4 (4707/7500) & 92.4 & 0.54 & 0.39 & 3.12 \\
& & & & Emilia (4733/7500) & 80.9 & 0.54 & 0.29 & 2.82 \\
& & & & Libri (4710/7500) & 63.4 & 0.49 & 0.36 & 2.86 \\

\midrule

\multirow{9}{*}{Llama-Mimi}
& \multirow{3}{*}{Emilia10k}
& \multirow{3}{*}{Matched reproduced}
& \multirow{3}{*}{241M}
& C4 (4707/7500) & 407.9 & 0.52 & 0.40 & 3.10 \\
& & & & Emilia (4733/7500) & 283.0 & 0.50 & 0.45 & 3.14 \\
& & & & Libri (4710/7500) & 328.3 & 0.55 & 0.38 & 2.94 \\

\addlinespace[2pt]

& \multirow{6}{*}{240k h speech}
& \multirow{6}{*}{Published}
& \multirow{3}{*}{973M}
& C4 (4707/7500) & 106.8 & 0.52 & 0.48 & 3.07 \\
& & & & Emilia (4733/7500) & 86.5 & 0.50 & 0.46 & 2.93 \\
& & & & Libri (4710/7500) & 80.0 & 0.47 & 0.44 & 2.92 \\
\cmidrule(lr){4-9}
& & & \multirow{3}{*}{7.54B}
& C4 (4707/7500) & 68.3 & 0.51 & 0.49 & 3.03 \\
& & & & Emilia (4733/7500) & 53.0 & 0.50 & 0.48 & 2.90 \\
& & & & Libri (4710/7500) & 48.7 & 0.47 & 0.45 & 2.92 \\

\bottomrule
\end{tabular}%
}
\end{table}

==> backup_intro.tex <==
Speech-text language models commonly introduce text either as an interleaved stream~\cite{chou2023toward,nguyen2025spirit} or as an internal representation~\cite{defossez2024moshi}. Recent scaling-law studies have also measured how speech language models improve with model size, data, and compute, for both textless models~\cite{cuervo2024scaling,ramapuram2026scaling} and interleaved speech-text models~\cite{maimon2025scaling}. These studies provide important evidence on how speech language modeling performance changes with scale, using metrics such as transcript-based generation quality, phonetic distributional measures, and downstream task performance. However, their goal is primarily to characterize scaling behavior rather than to decompose what aspects of generated speech are affected by text conditioning.

A related limitation is that many existing evaluations are tied to downstream tasks or post-training settings. While such evaluations are important, they make it difficult to isolate how the pre-training objective itself shapes generated speech. This is particularly relevant for speech-text language models, where improvements after post-training may reflect task adaptation or instruction tuning rather than the effect of text conditioning during pre-training. To understand the role of text in speech language modeling, we need a matched continuation protocol that compares speech-only, speech-text, and text-only models under the same generation setting and separates semantic, phonetic, and acoustic effects.


In this work, we study the speech–text modality gap as a controlled evaluation problem. We define the gap operationally: given matched prompts, how do speech-only, speech-text, and text-only language models differ when their continuations are evaluated through common projections? Text-only models provide a semantic comparison point in text space. Speech-only and speech-text models generate speech, which can be projected into text for semantic evaluation, into phones for local structure evaluation, and into acoustic or paralinguistic representations for speech-realization evaluation. This setup allows us to ask whether text conditioning makes generated speech closer to text-only continuations in semantic coherence, and whether such changes are also reflected in phone-level or acoustic-level metrics.

We propose a unified generation-based evaluation framework for this comparison. For semantic evaluation, text-only continuations are scored directly by a reference language model, while generated speech continuations are first transcribed and then scored by the same reference language model. This yields a transcript-based generation perplexity that can be compared across text-only, speech-only, and speech-text systems. For phonetic evaluation, we recognize phone sequences from generated speech and compare their local statistics with reference speech using phone n-gram divergence and entropy. For acoustic and paralinguistic evaluation, we compare speech-only and speech-text generations using automatic measures of quality, speaker consistency, and emotion consistency.

Using this framework, we find that text conditioning mainly improves the semantic projection of generated speech. Speech-text models achieve much lower transcript-based generation perplexity than speech-only models, indicating stronger linguistic coherence under the shared semantic evaluation. In contrast, local phone-statistic metrics show smaller differences between speech-only and speech-text generations, suggesting that the speech-only model already captures short-range phonetic structure reasonably well. Acoustic-related metrics show a different pattern: speech-only generations outperform speech-text generations, indicating that improvements in semantic coherence do not automatically translate into better acoustic or paralinguistic behavior. Training dynamics show a consistent pattern: the speech-text model first improves the text stream, after which the speech stream catches up, leading to faster overall convergence.

This work makes two main contributions. First, we introduce a matched continuation framework for comparing speech-only, speech-text, and text-only language models under a shared semantic evaluation, and extend it with phonetic and acoustic projections. Second, we use this framework to characterize the effect of text conditioning during speech language model pre-training, showing that text conditioning accelerates convergence and improves transcript-based semantic coherence, while local phone statistics change comparatively little and acoustic-related metrics favor speech-only models.

==> detailed_other.tex <==
% Requires \usepackage{booktabs,multirow,graphicx}
\begin{table*}[t]
\centering
\caption{Detailed continuation acoustic metrics under prompt-specific min-$k$ selection.}
\label{tab:llama-mimi-acoustic-metrics-detailed}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllcrrrrrrrrr@{}}
\toprule
 &  &  &  & \multicolumn{3}{c}{C4 prompts (4777/7500)} & \multicolumn{3}{c}{Emilia prompts (4780/7500)} & \multicolumn{3}{c}{Libri prompts (4855/7500)} \\
\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
Model & Training data & Variant & Params. & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ & pJSD $\downarrow$ & SpkSim $\uparrow$ & UTMOS $\uparrow$ \\
\midrule
\midrule
\multirow{6}{*}{Flow-based} & \multirow{2}{*}{C4} & Speech-only & 456M & 0.471 & 0.703 & 3.40 & 0.521 & 0.358 & 3.28 & 0.558 & 0.418 & 3.35 \\
 &  & Speech-text & 456M & 0.466 & 0.617 & 3.09 & 0.507 & 0.255 & 2.90 & 0.527 & 0.322 & 3.01 \\
\addlinespace[2pt]
 & \multirow{2}{*}{Emilia10k} & Speech-only & 456M & 0.537 & 0.441 & 3.34 & 0.511 & 0.466 & 3.19 & 0.558 & 0.399 & 3.11 \\
 &  & Speech-text & 456M & 0.532 & 0.360 & 3.23 & 0.503 & 0.411 & 3.07 & 0.545 & 0.330 & 3.03 \\
\addlinespace[2pt]
 & \multirow{2}{*}{MLSEn10k} & Speech-only & 456M & 0.566 & 0.533 & 3.43 & 0.549 & 0.417 & 3.22 & 0.496 & 0.494 & 3.23 \\
 &  & Speech-text & 456M & 0.539 & 0.393 & 3.12 & 0.539 & 0.291 & 2.82 & 0.486 & 0.360 & 2.86 \\
\midrule
\multirow{2}{*}{Llama-Mimi} & \multirow{2}{*}{240k h speech} & \multirow{2}{*}{Published} & 973M & 0.518 & 0.483 & 3.06 & 0.498 & 0.455 & 2.93 & 0.471 & 0.441 & 2.92 \\
 &  &  & 7.54B & 0.509 & 0.492 & 3.03 & 0.498 & 0.475 & 2.90 & 0.473 & 0.452 & 2.92 \\
\bottomrule
\end{tabular}%
}
\vspace{2pt}
\parbox{0.98\textwidth}{\footnotesize\emph{Note:} pJSD is the 5-gram phoneme Jensen--Shannon divergence. Speaker similarity compares the generated continuation with the full Mimi reference. Values are computed on the prompt-specific min-$k$ intersection across the eight displayed systems; metric means use available finite evaluator outputs, with metric-specific row counts reported in the companion TSV. Parameter counts exclude input embeddings.}
\end{table*}


==> detailed_table.tex <==
% Requires \usepackage{booktabs,multirow}
\begin{table*}[t]
\centering
\caption{Generation perplexity across training data and prompt domains.}
\label{tab:base-training-prompt-genppl}
\small
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lllcrrr@{}}
\toprule
 &  &  &  & \multicolumn{3}{c}{genPPL $\downarrow$ by prompt set} \\
\cmidrule(lr){5-7}
Model & Training data & Variant & Params. & \shortstack{C4\\(4707/7500)} & \shortstack{Emilia\\(4733/7500)} & \shortstack{Libri\\(4710/7500)} \\
\midrule
\midrule
\multirow{6}{*}{Flow-based} & \multirow{2}{*}{C4} & Speech-only & 456M & 228.8 & 265.1 & 291.6 \\
 &  & Speech-text & 456M & 49.9 & 51.8 & 63.4 \\
\addlinespace[2pt]
 & \multirow{2}{*}{Emilia10k} & Speech-only & 456M & 223.5 & 183.3 & 195.8 \\
 &  & Speech-text & 456M & 81.8 & 52.9 & 78.7 \\
\addlinespace[2pt]
 & \multirow{2}{*}{MLSEn10k} & Speech-only & 456M & 220.7 & 198.0 & 160.0 \\
 &  & Speech-text & 456M & 92.4 & 80.9 & 63.4 \\
\midrule
\multirow{3}{*}{Llama-Mimi} & Emilia10k & Matched reproduced & 241M & 407.9 & 283.0 & 328.3 \\
 & \multirow{2}{*}{240k h speech} & \multirow{2}{*}{Published} & 973M & 106.8 & 86.5 & 80.0 \\
 &  &  & 7.54B & 68.3 & 53.0 & 48.7 \\
\bottomrule
\end{tabular}
\vspace{2pt}
\parbox{0.98\textwidth}{\footnotesize\emph{Note:} Parentheses in the column headers report selected continuations out of 7,500. Prompt-set-specific min-$k$ is computed across exactly the nine displayed systems. Parameter counts exclude input embeddings. Speech-only and speech-text results use ASR transcriptions; internal text is excluded. The matched reproduced model uses Emilia10k and the same 40k-step budget as the flow-based base models.}
\end{table*}


==> tables/ppl.tex <==
% Auto-generated from results/batch_20260405_last_prompt1500_test_eval_subset_cond_ppl.tsv
% Requires \usepackage{booktabs}.

\begin{table}[t]
\centering
\small
\caption{Conditional perplexity on the min-$k$ matched continuation subset. For each prompt, $k$ is the minimum number of valid continuations across the nine systems; each system uses its first $k$ valid continuations.}
\label{tab:p1500-test-min-k-cond-ppl}
\begin{tabular}{llrrrrr}
\toprule
Prompt set & Train data & Text-only & Speech-only & Speech-text & Prompts & Cont. \\
\midrule
C4 & C4 & 31.7 & 228.5 & 48.7 & 1442 & 6234 \\
C4 & Emilia10k & 42.8 & 226.5 & 79.4 & 1442 & 6234 \\
C4 & MLSEn10k & 59.1 & 222.8 & 92.5 & 1442 & 6234 \\
\midrule
Emilia & C4 & 35.8 & 267.8 & 52.2 & 1425 & 6205 \\
Emilia & Emilia10k & 30.4 & 185.1 & 53.3 & 1425 & 6205 \\
Emilia & MLSEn10k & 47.1 & 197.5 & 80.7 & 1425 & 6205 \\
\midrule
LibriSpeech & C4 & 43.7 & 287.9 & 62.9 & 1477 & 6578 \\
LibriSpeech & Emilia10k & 41.5 & 196.4 & 76.1 & 1477 & 6578 \\
LibriSpeech & MLSEn10k & 36.5 & 160.0 & 62.8 & 1477 & 6578 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\small
\caption{Conditional perplexity on prompts where all nine systems have all five valid continuations.}
\label{tab:p1500-test-all-5-cond-ppl}
\begin{tabular}{llrrrrr}
\toprule
Prompt set & Train data & Text-only & Speech-only & Speech-text & Prompts & Cont. \\
\midrule
C4 & C4 & 30.9 & 228.0 & 47.2 & 895 & 4475 \\
C4 & Emilia10k & 41.4 & 222.2 & 75.9 & 895 & 4475 \\
C4 & MLSEn10k & 57.7 & 217.9 & 90.2 & 895 & 4475 \\
\midrule
Emilia & C4 & 35.6 & 267.8 & 52.3 & 915 & 4575 \\
Emilia & Emilia10k & 30.2 & 192.9 & 54.0 & 915 & 4575 \\
Emilia & MLSEn10k & 46.5 & 196.2 & 80.6 & 915 & 4575 \\
\midrule
LibriSpeech & C4 & 43.0 & 290.6 & 62.2 & 988 & 4940 \\
LibriSpeech & Emilia10k & 40.5 & 197.6 & 75.8 & 988 & 4940 \\
LibriSpeech & MLSEn10k & 36.0 & 159.5 & 62.6 & 988 & 4940 \\
\bottomrule
\end{tabular}
\end{table}

